Quantum nucleation of up-down quark matter and astrophysical implications

Quark matter with only $u$ and $d$ quarks ($ud$QM) might be the ground state of baryonic matter at large baryon number $A>A_{\rm min}$. With $A_{\rm min}\gtrsim 300$, this has no direct conflict with the stability of ordinary nuclei. An intriguing test of this scenario is to look for quantum nucleation of $ud$QM inside neutron stars due to their large baryon densities. In this paper, we study the transition rate of cold neutron stars to $ud$ quark stars ($ud$QSs) and the astrophysical implications, considering the relevant theoretical uncertainties and observational constraints. It turns out that a large portion of parameter space predicts an instantaneous transition, and so the observed neutron stars are mostly $ud$QSs. We find this possibility still viable under the recent gravitational wave and pulsar observations, although there are debates on its compatibility with some observations that involve complicated structure of quark matter. The tension could be partially relieved in the two-families scenario, where the high-mass stars ($M\gtrsim2 M_{\odot}$) are all $ud$QSs and the low-mass ones ($M\sim1.4\, M_{\odot}$) are mostly hadronic stars. In this case, the slow transition of the low-mass hadronic stars points to a very specific class of hadronic models with moderately stiff EOSs, and $ud$QM properties are also strongly constrained.

==> Transition v14/biblioTransition.tex <==

\bibitem{Bodmer:1971we} 
  A.~R.~Bodmer,
  %``Collapsed nuclei,''
  Phys.\ Rev.\ D {\bf 4}, 1601 (1971).
% doi:10.1103/PhysRevD.4.1601
%\cite{Holdom:2017gdc}
\bibitem{Witten}
%\bibitem{Witten:1984rs} 
  E.~Witten,
  %``Cosmic Separation of Phases,''
  Phys.\ Rev.\ D {\bf 30}, 272 (1984).
% doi:10.1103/PhysRevD.30.272
\bibitem{Terazawa:1979hq} 
  H.~Terazawa,
 % ``Quark Shell Model And Superheavy Hypernucleus,''
  INS-Report-336 (INS, University of Tokyo, Tokyo) May, 1979.
  %\cite{Wang:2002pza}
  %\cite{Buballa:1998pr}

  \bibitem{HRZ2017}
  B.~Holdom, J.~Ren and C.~Zhang,
  %``Quark matter may not be strange,''
  Phys.\ Rev.\ Lett.\  {\bf 120} (2018) no.22,  222001
  doi:10.1103/PhysRevLett.120.222001
  [arXiv:1707.06610 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevLett.120.222001;%%
  %1 citations counted in INSPIRE as of 02 Aug 2018
%\cite{Iida:2020fyt}
\bibitem{Iida:2020fyt}
K.~Iida and T.~Fujie,
%``On the Stability of Giant Nuclei in Supernova Matter with Respect to Deconfinement,''
JPS Conf. Proc. \textbf{31}, 011057 (2020)
doi:10.7566/JPSCP.31.011057
%0 citations counted in INSPIRE as of 09 Jun 2020
%\cite{Xia:2020byy}


%\cite{Burdin:2014xma}
\bibitem{Burdin:2014xma}
S.~Burdin, M.~Fairbairn, P.~Mermod, D.~Milstead, J.~Pinfold, T.~Sloan and W.~Taylor,
%``Non-collider searches for stable massive particles,''
Phys. Rept. \textbf{582}, 1-52 (2015)
doi:10.1016/j.physrep.2015.03.004
[arXiv:1410.1374 [hep-ph]].
%60 citations counted in INSPIRE as of 24 May 2020

\bibitem{Sandweiss:2004bu}
J.~Sandweiss,
%``Overview of strangelet searches and Alpha Magnetic Spectrometer: When will we stop searching?,''
J. Phys. G \textbf{30}, S51-S59 (2004)
doi:10.1088/0954-3899/30/1/004

\bibitem{Aad:2019pfm} 
  G.~Aad {\it et al.} [ATLAS Collaboration],
  %``Search for magnetic monopoles and stable high-electric-charge objects in 13 TeV proton-proton collisions with the ATLAS detector,''
  arXiv:1905.10130 [hep-ex].
  %%CITATION = ARXIV:1905.10130;%%
  %3 citations counted in INSPIRE as of 24 Aug 2019

\bibitem{Xia:2020byy}
C.~J.~Xia, S.~S.~Xue, R.~X.~Xu and S.~G.~Zhou,
%``Supercritical charged objects and $e^+e^-$ pair creation,''
Phys. Rev. D \textbf{101}, no.10, 103031 (2020)
doi:10.1103/PhysRevD.101.103031
[arXiv:2001.03531 [nucl-th]].
%0 citations counted in INSPIRE as of 09 Jun 2020
%\cite{Aad:2019pfm}


\bibitem{Demorest:2010bx} 
  P.~Demorest, T.~Pennucci, S.~Ransom, M.~Roberts and J.~Hessels,
  %``Shapiro Delay Measurement of A Two Solar Mass Neutron Star,''
  Nature {\bf 467}, 1081 (2010)
  doi:10.1038/nature09466
  [arXiv:1010.5788 [astro-ph.HE]].
  %%CITATION = doi:10.1038/nature09466;%%
  %2040 citations counted in INSPIRE as of 17 Sep 2019
%\cite{Antoniadis:2013pzd}

%\cite{Cromartie:2019kug}
\bibitem{Cromartie:2019kug} 
  H.~T.~Cromartie {\it et al.},
  %``Relativistic Shapiro delay measurements of an extremely massive millisecond pulsar,''
  doi:10.1038/s41550-019-0880-2
  arXiv:1904.06759 [astro-ph.HE].
  %%CITATION = doi:10.1038/s41550-019-0880-2;%%
  %63 citations counted in INSPIRE as of 17 Sep 2019

\bibitem{Antoniadis:2013pzd}
J.~Antoniadis, P.~C.~Freire, N.~Wex, T.~M.~Tauris, R.~S.~Lynch, M.~H.~van Kerkwijk, M.~Kramer, C.~Bassa, V.~S.~Dhillon, T.~Driebe, J.~W.~Hessels, V.~M.~Kaspi, V.~I.~Kondratiev, N.~Langer, T.~R.~Marsh, M.~A.~McLaughlin, T.~T.~Pennucci, S.~M.~Ransom, I.~H.~Stairs, J.~van Leeuwen, J.~P.~Verbiest and D.~G.~Whelan,
%``A Massive Pulsar in a Compact Relativistic Binary,''
Science \textbf{340}, 6131 (2013)
doi:10.1126/science.1233232
[arXiv:1304.6875 [astro-ph.HE]].


%\cite{Xu:2007wd}

    \bibitem{Drago:2013fsa} 
  A.~Drago, A.~Lavagno and G.~Pagliara,
  %``Can very compact and very massive neutron stars both exist?,''
  Phys.\ Rev.\ D {\bf 89}, no. 4, 043014 (2014)
  doi:10.1103/PhysRevD.89.043014
  [arXiv:1309.7263 [nucl-th]].
  %%CITATION = doi:10.1103/PhysRevD.89.043014;%%
  %73 citations counted in INSPIRE as of 27 Aug 2019
%\cite{Drago:2017bnf}
%\cite{Zacchi:2015lwa}
\bibitem{Zacchi:2015lwa}
A.~Zacchi, R.~Stiele and J.~Schaffner-Bielich,
%``Compact stars in a SU(3) Quark-Meson Model,''
Phys. Rev. D \textbf{92}, no.4, 045022 (2015)
doi:10.1103/PhysRevD.92.045022
[arXiv:1506.01868 [astro-ph.HE]].
%28 citations counted in INSPIRE as of 18 May 2020
%\cite{Burgio:2018yix}

%\cite{Bombaci:2016xuj}
\bibitem{Bombaci:2016xuj}
I.~Bombaci, D.~Logoteta, I.~Vidaña and C.~Providência,
%``Quark matter nucleation in neutron stars and astrophysical implications,''
Eur. Phys. J. A \textbf{52}, no.3, 58 (2016)
doi:10.1140/epja/i2016-16058-5
[arXiv:1601.04559 [astro-ph.HE]].
%31 citations counted in INSPIRE as of 18 May 2020

%\cite{Zhou:2017pha}
\bibitem{Zhou:2017pha}
E.~P.~Zhou, X.~Zhou and A.~Li,
%``Constraints on interquark interaction parameters with GW170817 in a binary strange star scenario,''
Phys. Rev. D \textbf{97}, no.8, 083015 (2018)
doi:10.1103/PhysRevD.97.083015
[arXiv:1711.04312 [astro-ph.HE]].
\bibitem{Burgio:2018yix}
G.~Burgio, A.~Drago, G.~Pagliara, H.~J.~Schulze and J.~B.~Wei,
%``Are Small Radii of Compact Stars Ruled out by GW170817/AT2017gfo?,''
Astrophys. J. \textbf{860}, no.2, 139 (2018)
doi:10.3847/1538-4357/aac6ee
[arXiv:1803.09696 [astro-ph.HE]].
%51 citations counted in INSPIRE as of 04 Jun 2020



%\cite{Zhang:2019mqb}
\bibitem{Zhang:2019mqb}
C.~Zhang,
%``Probing up-down quark matter via gravitational waves,''
Phys. Rev. D \textbf{101}, no.4, 043003 (2020)
doi:10.1103/PhysRevD.101.043003
[arXiv:1908.10355 [astro-ph.HE]].
%2 citations counted in INSPIRE as of 18 Apr 2020
%\cite{Wang:2019jze}
\bibitem{Zhao:2019xqy} 
  T.~Zhao, W.~Zheng, F.~Wang, C.~M.~Li, Y.~Yan, Y.~F.~Huang and H.~S.~Zong,
  %``Do current astronomical observations exclude the existence of nonstrange quark stars?,''
  Phys.\ Rev.\ D {\bf 100}, no. 4, 043018 (2019)
  doi:10.1103/PhysRevD.100.043018
  [arXiv:1904.09744 [nucl-th]].
  %%CITATION = doi:10.1103/PhysRevD.100.043018;%%
  %2 citations counted in INSPIRE as of 10 Sep 2019

\bibitem{Xu:2007wd} 
  R.~Xu,
  %``Possible evidence that pulsars are quark stars,''
  AIP Conf.\ Proc.\  {\bf 968}, no. 1, 197 (2008)
  doi:10.1063/1.2840396
  [arXiv:0709.1305 [astro-ph]].
  %%CITATION = doi:10.1063/1.2840396;%%
  %8 citations counted in INSPIRE as of 28 Dec 2019
\bibitem{Wang:2019jze}
Q.~Wang, C.~Shi and H.~Zong,
%``Nonstrange quark stars from an NJL model with proper-time regularization,''
Phys. Rev. D \textbf{100}, no.12, 123003 (2019)
doi:10.1103/PhysRevD.100.123003
[arXiv:1908.06558 [hep-ph]].
%5 citations counted in INSPIRE as of 22 Apr 2020

%\cite{Abbott:2020uma}
\bibitem{Abbott:2020uma}
B.~Abbott \textit{et al.} [LIGO Scientific and Virgo],
%``GW190425: Observation of a Compact Binary Coalescence with Total Mass $\sim 3.4 M_{\odot}$,''
Astrophys. J. Lett. \textbf{892}, L3 (2020)
doi:10.3847/2041-8213/ab75f5
[arXiv:2001.01761 [astro-ph.HE]].
%73 citations counted in INSPIRE as of 17 Apr 2020
\bibitem{Wen:2010zz}
X.~Wen, J.~Li, J.~Liang and G.~Peng,
%``Medium effects on the surface tension of strangelets in the extended quasiparticle model,''
Phys. Rev. C \textbf{82}, 025809 (2010)
doi:10.1103/PhysRevC.82.025809
%22 citations counted in INSPIRE as of 07 May 2020
%\cite{Most:2019onn}
\bibitem{Dexheimer:2019pay}
V.~Dexheimer, L.~Soethe, J.~Roark, R.~Gomes, S.~Kepler and S.~Schramm,
%``Phase Transitions in Neutron Stars,''
Int. J. Mod. Phys. E \textbf{27}, no.11, 1830008 (2018)
doi:10.1142/S0218301318300084
[arXiv:1901.03252 [astro-ph.HE]].
%5 citations counted in INSPIRE as of 09 Jun 2020

\bibitem{Most:2019onn}
E.~R.~Most, L.~Jens Papenfort, V.~Dexheimer, M.~Hanauske, H.~Stoecker and L.~Rezzolla,
%``On the deconfinement phase transition in neutron-star mergers,''
Eur. Phys. J. A \textbf{56}, no.2, 59 (2020)
doi:10.1140/epja/s10050-020-00073-4
[arXiv:1910.13893 [astro-ph.HE]].
%7 citations counted in INSPIRE as of 09 Jun 2020
%\cite{Dexheimer:2019pay}



  %\cite{Weissenborn:2011qu}
\bibitem{Weissenborn:2011qu} 
  S.~Weissenborn, I.~Sagert, G.~Pagliara, M.~Hempel and J.~Schaffner-Bielich,
  %``Quark Matter In Massive Neutron Stars,''
  Astrophys.\ J.\  {\bf 740}, L14 (2011)
  doi:10.1088/2041-8205/740/1/L14
  [arXiv:1102.2869 [astro-ph.HE]].
  %%CITATION = doi:10.1088/2041-8205/740/1/L14;%%
  %152 citations counted in INSPIRE as of 13 Aug 2019
  
\bibitem{Tolman:1939jz} 
  R.~C.~Tolman,
  %``Static solutions of Einstein's field equations for spheres of fluid,''
  Phys.\ Rev.\  {\bf 55}, 364 (1939).
  doi:10.1103/PhysRev.55.364
  %%CITATION = doi:10.1103/PhysRev.55.364;%%
  %1050 citations counted in INSPIRE as of 30 Sep 2019
  
\bibitem{Oppenheimer:1939ne} 
  J.~R.~Oppenheimer and G.~M.~Volkoff,
  %``On Massive neutron cores,''
  Phys.\ Rev.\  {\bf 55}, 374 (1939).
  doi:10.1103/PhysRev.55.374
  %%CITATION = doi:10.1103/PhysRev.55.374;%%
  %1501 citations counted in INSPIRE as of 30 Sep 2019


\bibitem{Zdunik:2000xx} 
  J.~L.~Zdunik,
  %``Strange stars: Linear approximation of the EOS and maximum QPO frequency,''
  Astron.\ Astrophys.\  {\bf 359}, 311 (2000)
  [astro-ph/0004375].
  %%CITATION = ASTRO-PH/0004375;%%
  %50 citations counted in INSPIRE as of 21 Aug 2019
\bibitem{Haensel:2007yy} 
  P.~Haensel, A.~Y.~Potekhin and D.~G.~Yakovlev,
  %``Neutron stars 1: Equation of state and structure,''
  Astrophys.\ Space Sci.\ Libr.\  {\bf 326}, pp.1 (2007).
  doi:10.1007/978-0-387-47301-7
  
%\cite{Linares:2018ppq}
\bibitem{Linares:2018ppq}
M.~Linares, T.~Shahbaz and J.~Casares,
%``Peering into the dark side: Magnesium lines establish a massive neutron star in PSR J2215+5135,''
Astrophys. J. \textbf{859}, no.1, 54 (2018)
doi:10.3847/1538-4357/aabde6
[arXiv:1805.08799 [astro-ph.HE]].
%64 citations counted in INSPIRE as of 21 May 2020


%\cite{TheLIGOScientific:2017qsa}
\bibitem{TheLIGOScientific:2017qsa}
B.~Abbott \textit{et al.} [LIGO Scientific and Virgo],
%``GW170817: Observation of Gravitational Waves from a Binary Neutron Star Inspiral,''
Phys. Rev. Lett. \textbf{119}, no.16, 161101 (2017)
doi:10.1103/PhysRevLett.119.161101
[arXiv:1710.05832 [gr-qc]].
%3114 citations counted in INSPIRE as of 17 Apr 2020
  \bibitem{Abbott:2018wiz} 
  B.~P.~Abbott {\it et al.} [LIGO Scientific and Virgo Collaborations],
  %``Properties of the binary neutron star merger GW170817,''
  Phys.\ Rev.\ X {\bf 9}, no. 1, 011001 (2019)
  doi:10.1103/PhysRevX.9.011001
  [arXiv:1805.11579 [gr-qc]].
  
  



%%%%%%
\bibitem{lk72}   I.M. Lifshitz, Y. Kagan, {\it Sov. Phys. JETP} {\bf 35}, 206 (1972).   

\bibitem{iida98}  K. Iida, K. Sato, {\it Phys. Rev.} C {\bf 58}, 2538 (1998).  
\bibitem{LK} I. M. Lifshitz and Yu.\ Kagan, Zh.\ Eksp.\ Teor.\ Fiz.\ 
{\bf 62}, 385 (1972) [Sov.\ Phys.\ JETP {\bf 35}, 206 (1972)].
 \bibitem{Berger:1986ps} 
  M.~S.~Berger and R.~L.~Jaffe,
  %``Radioactivity in strange quark matter,''
  Phys.\ Rev.\ C {\bf 35}, 213 (1987).
% doi:10.1103/PhysRevC.35.213
 

  
  %\cite{Ke:2013wga}
\bibitem{Ke:2013wga} 
  W.~y.~Ke and Y.~x.~Liu,
  %``Interface tension and interface entropy in the 2+1 flavor Nambu-Jona-Lasinio model,''
  Phys.\ Rev.\ D {\bf 89}, no. 7, 074041 (2014)
  doi:10.1103/PhysRevD.89.074041
  [arXiv:1312.2295 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.89.074041;%%
  %18 citations counted in INSPIRE as of 12 Aug 2019
  %\cite{Garcia:2013eaa}
\bibitem{Garcia:2013eaa} 
  A.~F.~Garcia and M.~B.~Pinto,
  %``Surface tension of magnetized quark matter,''
  Phys.\ Rev.\ C {\bf 88}, no. 2, 025207 (2013)
  doi:10.1103/PhysRevC.88.025207
  [arXiv:1306.3090 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevC.88.025207;%%
  %22 citations counted in INSPIRE as of 12 Aug 2019
  %\cite{Voskresensky:2002hu}
  %\cite{Fraga:2018cvr}
  
  

  
\bibitem{Palhares:2010be} 
  L.~F.~Palhares and E.~S.~Fraga,
  %``Droplets in the cold and dense linear sigma model with quarks,''
  Phys.\ Rev.\ D {\bf 82}, 125018 (2010)
  doi:10.1103/PhysRevD.82.125018
  [arXiv:1006.2357 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.82.125018;%%
  %61 citations counted in INSPIRE as of 12 Aug 2019
  %\cite{Pinto:2012aq}

\bibitem{Pinto:2012aq} 
  M.~B.~Pinto, V.~Koch and J.~Randrup,
  %``The Surface Tension of Quark Matter in a Geometrical Approach,''
  Phys.\ Rev.\ C {\bf 86}, 025203 (2012)
  doi:10.1103/PhysRevC.86.025203
  [arXiv:1207.5186 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevC.86.025203;%%
  %62 citations counted in INSPIRE as of 12 Aug 2019
  
\bibitem{Fraga:2018cvr} 
  E.~S.~Fraga, M.~Hippert and A.~Schmitt,
  %``Surface tension of dense matter at the chiral phase transition,''
  Phys.\ Rev.\ D {\bf 99}, no. 1, 014046 (2019)
  doi:10.1103/PhysRevD.99.014046
  [arXiv:1810.13226 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.99.014046;%%
  %5 citations counted in INSPIRE as of 12 Aug 2019
  
\bibitem{Lugones:2013ema} 
  G.~Lugones, A.~G.~Grunfeld and M.~Al Ajmi,
  %``Surface tension and curvature energy of quark matter in the Nambu-Jona-Lasinio model,''
  Phys.\ Rev.\ C {\bf 88}, no. 4, 045803 (2013)
  doi:10.1103/PhysRevC.88.045803
  [arXiv:1308.1452 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevC.88.045803;%%
  %41 citations counted in INSPIRE as of 12 Aug 2019  
  
\bibitem{Voskresensky:2002hu} 
  D.~N.~Voskresensky, M.~Yasuhira and T.~Tatsumi,
  %``Charge screening at first order phase transitions and hadron quark mixed phase,''
  Nucl.\ Phys.\ A {\bf 723}, 291 (2003)
  doi:10.1016/S0375-9474(03)01313-7
  [nucl-th/0208067].


%%%%%%%%%%%%%%%%%

 \bibitem{ucm_nEOS}  http://teorica.fis.ucm.es/nEOS/
 
 \bibitem{Compose}https://compose.obspm.fr/
 
 
 %\cite{Landry:2020vaw}
\bibitem{Landry:2020vaw}
P.~Landry, R.~Essick and K.~Chatziioannou,
%``Nonparametric constraints on neutron star matter with existing and upcoming gravitational wave and pulsar observations,''
[arXiv:2003.04880 [astro-ph.HE]].
%0 citations counted in INSPIRE as of 01 Apr 2020
  
\bibitem{Riley:2019yda}
T.~E.~Riley, A.~L.~Watts, S.~Bogdanov, P.~S.~Ray, R.~M.~Ludlam, S.~Guillot, Z.~Arzoumanian, C.~L.~Baker, A.~V.~Bilous, D.~Chakrabarty, K.~C.~Gendreau, A.~K.~Harding, W.~C.~Ho, J.~M.~Lattimer, S.~M.~Morsink and T.~E.~Strohmayer,
%``A $NICER$ View of PSR J0030+0451: Millisecond Pulsar Parameter Estimation,''
Astrophys. J. Lett. \textbf{887}, no.1, L21 (2019)
doi:10.3847/2041-8213/ab481c
[arXiv:1912.05702 [astro-ph.HE]].
%49 citations counted in INSPIRE as of 06 May 2020

\bibitem{Miller:2019cac}
M.~Miller, F.~Lamb, A.~Dittmann, S.~Bogdanov, Z.~Arzoumanian, K.~Gendreau, S.~Guillot, A.~Harding, W.~Ho, J.~Lattimer, R.~Ludlam, S.~Mahmoodifar, S.~Morsink, P.~Ray, T.~Strohmayer, K.~Wood, T.~Enoto, R.~Foster, T.~Okajima, G.~Prigozhin and Y.~Soong,
%``PSR J0030+0451 Mass and Radius from $NICER$ Data and Implications for the Properties of Neutron Star Matter,''
Astrophys. J. Lett. \textbf{887}, no.1, L24 (2019)
doi:10.3847/2041-8213/ab50c5
[arXiv:1912.05705 [astro-ph.HE]].
%50 citations counted in INSPIRE as of 06 May 2020
  
%\cite{Anderson:1975zze}
\bibitem{Anderson:1975zze}
P.~Anderson and N.~Itoh,
%``Pulsar glitches and restlessness as a hard superfluidity phenomenon,''
Nature \textbf{256}, 25-27 (1975)
doi:10.1038/256025a0
%400 citations counted in INSPIRE as of 11 May 2020

\bibitem{Alpar:1977}
M. A.~Alpar, 
Astrophys. J. 213, 527 (1977)
doi:10.1038/256025a0

%\cite{Alpar:1987vk}
\bibitem{Alpar:1987vk}
M.~Alpar,
%``COMMENT ON STRANGE STARS,''
Phys. Rev. Lett. \textbf{58}, 2152 (1987)
doi:10.1103/PhysRevLett.58.2152
%85 citations counted in INSPIRE as of 17 Apr 2020


%\cite{Glendenning:1992kd}
\bibitem{Glendenning:1992kd}
N.~Glendenning and F.~Weber,
%``Nuclear solid crust on rotating strange quark stars,''
Astrophys. J. \textbf{400}, 647-658 (1992)
doi:10.1086/172026
%128 citations counted in INSPIRE as of 17 Apr 2020

 
 

 
%\cite{Alcock:1986hz}
\bibitem{Alcock:1986hz}
C.~Alcock, E.~Farhi and A.~Olinto,
%``Strange stars,''
Astrophys. J. \textbf{310}, 261-272 (1986)
doi:10.1086/164679
%856 citations counted in INSPIRE as of 17 Apr 2020
 
 
%\cite{Jaikumar:2005ne}
\bibitem{Jaikumar:2005ne}
P.~Jaikumar, S.~Reddy and A.~W.~Steiner,
%``The Strange star surface: A Crust with nuggets,''
Phys. Rev. Lett. \textbf{96}, 041101 (2006)
doi:10.1103/PhysRevLett.96.041101
[arXiv:nucl-th/0507055 [nucl-th]]. 

\bibitem{Anglani:2013gfu} 
  R.~Anglani, R.~Casalbuoni, M.~Ciminale, N.~Ippolito, R.~Gatto, M.~Mannarelli and M.~Ruggieri,
  %``Crystalline color superconductors,''
  Rev.\ Mod.\ Phys.\  {\bf 86}, 509 (2014)
  %doi:10.1103/RevModPhys.86.509
  [arXiv:1302.4264 [hep-ph]].
  %%CITATION = doi:10.1103/RevModPhys.86.509;%%
  %94 citations counted in INSPIRE as of 01 Oct 2019

%\cite{Watts:2006hk}
\bibitem{Watts:2006hk}
A.~L.~Watts and S.~Reddy,
%``Magnetar oscillations pose challenges for strange stars,''
Mon. Not. Roy. Astron. Soc. \textbf{379}, L63 (2007)
doi:10.1111/j.1745-3933.2007.00336.x
[arXiv:astro-ph/0609364 [astro-ph]].

%\cite{Miller:2018kmk}
\bibitem{Miller:2018kmk}
M.~C.~Miller, C.~Chirenti and T.~Strohmayer,
%``On the Persistence of QPOs During the SGR 1806-20 Giant Flare,''
Astrophys. J. \textbf{871}, 95 (2019)
doi:10.3847/1538-4357/aaf5ce
[arXiv:1808.09483 [astro-ph.HE]].



\bibitem{Bauswein:2008gx}
A.~Bauswein, H.~Janka, R.~Oechslin, G.~Pagliara, I.~Sagert, J.~Schaffner-Bielich, M.~Hohle and R.~Neuhauser,
%``Mass Ejection by Strange Star Mergers and Observational Implications,''
Phys. Rev. Lett. \textbf{103}, 011101 (2009)
doi:10.1103/PhysRevLett.103.011101
[arXiv:0812.4248 [astro-ph]].
%70 citations counted in INSPIRE as of 23 Apr 2020

%%%%%%%%%%%%%%%%%%%%%%%%


  \bibitem{AELove} A. E. H. Love, Proc. R. Soc. A 82, 73 (1909).
    \bibitem{Hinderer:2007mb} 
  T.~Hinderer,
  %``Tidal Love numbers of neutron stars,''
  Astrophys.\ J.\  {\bf 677}, 1216 (2008)
  doi:10.1086/533487
  [arXiv:0711.2420 [astro-ph]].
  %%CITATION = doi:10.1086/533487;%%
 %\cite{Hinderer:2009ca}
\bibitem{Hinderer:2009ca} 
  T.~Hinderer, B.~D.~Lackey, R.~N.~Lang and J.~S.~Read,
  %``Tidal deformability of neutron stars with realistic equations of state and their gravitational wave signatures in binary inspiral,''
  Phys.\ Rev.\ D {\bf 81}, 123016 (2010)
  doi:10.1103/PhysRevD.81.123016
  [arXiv:0911.3535 [astro-ph.HE]].

  \bibitem{Postnikov:2010yn} 
  S.~Postnikov, M.~Prakash and J.~M.~Lattimer,
  %``Tidal Love Numbers of Neutron and Self-Bound Quark Stars,''
  Phys.\ Rev.\ D {\bf 82}, 024016 (2010)
  doi:10.1103/PhysRevD.82.024016
  [arXiv:1004.5098 [astro-ph.SR]].
  %%CITATION = doi:10.1103/PhysRevD.82.024016;%%


 \bibitem{Damour:2009vw} 
  T.~Damour and A.~Nagar,
  %``Relativistic tidal properties of neutron stars,''
  Phys.\ Rev.\ D {\bf 80}, 084035 (2009)
  doi:10.1103/PhysRevD.80.084035
  [arXiv:0906.0096 [gr-qc]].


%%%%%%%%%%%%%%%

  

